An Empirical Study of Static Analysis Tools for Secure Code Review

Early identification of security issues in software development is vital to minimize their unanticipated impacts. Code review is a widely used manual analysis method that aims to uncover security issues along with other coding issues in software projects. While some studies suggest that automated static application security testing tools (SASTs) could enhance security issue identification, there is limited understanding of SAST's practical effectiveness in supporting secure code review. Moreover, most SAST studies rely on synthetic or fully vulnerable versions of the subject program, which may not accurately represent real-world code changes in the code review process. To address this gap, we study C/C++ SASTs using a dataset of actual code changes that contributed to exploitable vulnerabilities. Beyond SAST's effectiveness, we quantify potential benefits when changed functions are prioritized by SAST warnings. Our dataset comprises 319 real-world vulnerabilities from 815 vulnerability-contributing commits (VCCs) in 92 C and C++ projects. The result reveals that a single SAST can produce warnings in vulnerable functions of 52% of VCCs. Prioritizing changed functions with SAST warnings can improve accuracy (i.e., 12% of precision and 5.6% of recall) and reduce Initial False Alarm (lines of code in non-vulnerable functions inspected until the first vulnerable function) by 13%. Nevertheless, at least 76% of the warnings in vulnerable functions are irrelevant to the VCCs, and 22% of VCCs remain undetected due to limitations of SAST rules. Our findings highlight the benefits and the remaining gaps of SAST-supported secure code reviews and challenges that should be addressed in future work.

==> section/analysis_details.tex <==
\subsection{Detection Scenarios}
We define the scenarios in which the tools can detect the vulnerabilities based on two aspects: \textcircled{1} the granularity of changes that receive warnings and \textcircled{2} the type of vulnerability in the warnings. 
We combine the detection scenarios from the previous works~\cite{Thung2012ToTools, Lipp2022AnDetection, Li2023ComparisonJava} by including file-level detection and the number of warned changes because we want to understand the tool's performance from a broader perspective.
We consider the effectiveness of the tools in the eight following detection scenarios.

\begin{itemize}
    \item \textbf{Scenario F-A:} At least one vulnerable file receives the warnings
    \item \textbf{Scenario F-B:} At least one vulnerable file receives the warnings with the correct vulnerability type
    \item \textbf{Scenario F-C:} All vulnerable files receive the warnings
    \item \textbf{Scenario F-D:} All vulnerable files receive the warnings with the correct vulnerability type
    \item \textbf{Scenario FN-A:} At least one vulnerable function receives the warnings
    \item \textbf{Scenario FN-B:} At least one vulnerable function receives the warnings with the correct vulnerability type
    \item \textbf{Scenario FN-C:} All vulnerable functions receive the warnings
    \item \textbf{Scenario FN-D:} All vulnerable functions receive the warnings with the correct vulnerability type
\end{itemize}

\inlineheading{Code Change Granularity} - Two granularities in code changes are analyzed in this study: \textcircled{1} File and \textcircled{2} Function. We do not match the warnings with vulnerable changes at line level because prior work~\cite{Lipp2022AnDetection} showed that similar warnings from different \SAT{} can appear in different locations in the code.





\subsection{Analysis Metrics}
We explain the metrics for \textcircled{1} tool's effectiveness, \textcircled{2} code review performance, and \textcircled{3} computation time in this section.

\inlineheading{Tool Effectiveness} - We analyze the proportion of detected VCCs in each scenario described in the previous section. 
The percentage of detected VCCs indicates how effectively a tool can detect potential vulnerabilities in different scenarios.
Hence, we use the percentage of the detected VCCs in each scenario to analyze the effectiveness of the tools.
Additionally, we also investigate the types of vulnerabilities that the tools can correctly produce the warnings at the function level (i.e., Scenario FN-D). 



==> section/data_preparation_details.tex <==

\inlineheading{1) Identify VCC's programming language}:
% As we aim to study C and C++ \SAT{s}, 
We select VCCs from the projects that are implemented in C and C++.
However, the original VCC dataset does not distinguish the programming languages of the VCCs.
To identify the VCC's programming language, we obtain the main programming language used by each project from GitHub API.
This step excludes \textcolor{red}{6,499} VCCs in \textcolor{red}{678} projects from the original VCC dataset. 

\inlineheading{2) Examine the types of vulnerabilities}:
% The type of vulnerability related to the VCC is required for our study.
CVE vulnerability is assigned a vulnerability type in the Common Weakness Enumeration (CWE) taxonomy. 
However, we notice that some vulnerabilities in the VCC dataset may have insufficient vulnerability type information.
We apply this criterion to ensure that the selected VCCs can be linked to at least one type of vulnerability.

To determine the vulnerability type of a VCC, we review the VCCs from Step 1.
We exclude \textcolor{red}{339} VCCs associated with \textcolor{red}{114} vulnerabilities that are not assigned with any CWE items.
For example, VCCs that contributed to CVE-2016-8677\footnote{\url{https://nvd.nist.gov/vuln/detail/CVE-2016-8677}} are excluded because the record does not have CWE information.
All remaining VCCs are related to the vulnerabilities that have been assigned with at least one CWE item.

\inlineheading{3) Verify if VCCs can be analyzed by \SAT{s}}:
Some \SAT{s} analyze the VCCs based on the information from the compilation process.
It is infeasible to test the compilation of all remaining VCCs.
We review the documents of the remaining projects to understand the preferred compilation procedure and classify the projects into three groups: \textcircled{1} projects that use the standard build process i.e., \texttt{automake}, \textcircled{2} projects that use the other automated build processes e.g., \texttt{cmake} and \texttt{meson}, and 3) projects that do not use automated build process or do not specify the preferred build process.
% We also collect the required dependencies for each project.
To facilitate our analysis, we select the projects from the first group to continue our study.
We exclude \textcolor{red}{3,519} VCCs from \textcolor{red}{212} projects.
Additionally, we execute the compilation test for the remaining VCCs.
We exclude other \textcolor{red}{491} VCCs that cannot be compiled in this step.

To compile the VCCs, we update \texttt{Makefile} by running the automated script that the projects have prepared for the compilation i.e., \texttt{autogen.sh}, \texttt{bootstrap.sh}, and \texttt{build.sh}.If none of the scripts is present, we use the \texttt{autoreconf} command to generate the required files.
Then, we run the configuration file i.e., \texttt{configure}.
Finally, we compile the program using \texttt{make -i} command. Note that we also use this procedure for \SAT{} execution.


==> table/table-consequence-scenario-distribution.tex <==


\begin{table}[ht!]
\centering
\small
\begin{tabularx}{\linewidth}{
            >{\hsize=0.2\hsize}X
            >{\hsize=2.0\hsize}X
            >{\hsize=0.9\hsize}X
            >{\hsize=0.9\hsize}X
          }
\toprule

   \multicolumn{2}{c}{\textbf{Consequence scenario}} & \textbf{OpenSSL} & \textbf{PHP}\\
  & & #(\%) & #(\%) \\
  \hline
\multirow{2}{*}{ \textbf{C1}} & C1.1: Successfully fixed & xx (xx\%)  & 35 (29\%)\\
                              & C1.2: Unsuccessfully fixed & xx (xx\%)  & 14 (11\%)\\
 \cline{2-4}
\multirow{2}{*}{ \textbf{C2}} & C2.1: To fix elsewhere & xx (xx\%)  & 22 (18\%)\\
                              & C2.2: Un-resolved & xx (xx\%)  & 22 (18\%) \\
 \cline{2-4}
\multirow{2}{*}{ \textbf{C3}} & C3.1: False concern & xx (xx\%)  & 9 (7\%) \\
                              & C3.2: Design choice & xx (xx\%)  & 8 (6\%) \\
 \cline{2-4}
\multirow{2}{*}{ \textbf{C4}} & C4.1: Redundant & xx (xx\%)  & 4 (3\%)\\
                              & C4.2: Out of context & --  & 2 (2\%) \\
                              & C4.3: Unknown & xx (xx\%)  & 4 (3\%)  \\
 \bottomrule
\end{tabularx}
\newline
\caption{Detailed scenario distribution of security-related comments. The complete data set, including scenario distribution by category, can be found in the data release package. }
\label{table:consequence_scenario_distribution}
\vspace{-6mm}
\end{table}

==> table/table-original-vcc-dataset.tex <==
\begin{table}[h]
\centering
\small
\caption{Original and Selected Vulnerability Contributing Commits (VCCs)}
\begin{tabularx}{\linewidth}{
            >{\hsize=1.4\hsize}X
            >{\hsize=.8\hsize}X
            >{\hsize=.8\hsize}X
          }
\toprule
\textbf{Description} & \textbf{Original} &  \textbf{Selected} \\
 \midrule
 Commits & 11,853 & 815  \\ 
 Projects & 1,019  & 92 \\
 Programming Languages & 39   & 2 \\ 
 Vulnerabilities & 3,056  & 319 \\ 
 \bottomrule
\end{tabularx}
\newline
\label{table:original-vcc-dataset}
\end{table}

==> table/table-pull-request-consequences.tex <==
\begin{table}[ht!]
\centering
\small
\caption{Consequences of security-related comments}
\begin{tabularx}{\linewidth}{
            >{\hsize=2\hsize}X
            >{\hsize=0.5\hsize}X
            >{\hsize=0.5\hsize}X
          }
\toprule
 \multirow{2}{*}{\textbf{Security Concern's Consequence}} & \textbf{OpenSSL} &\textbf{ PHP}  \\
 & Comments & Comments \\
 \midrule
 C1: Developer attempted to fix the issue & xx (xx\%) & 49 (40\%) \\ 
 C2: Problem was acknowledged & xx (xx\%) & 44 (36\%) \\ 
 C3: Problem was dismissed  & xx (xx\%) & 17 (14\%) \\ 
 C4: Neither acknowledged nor fixed & xx (xx\%) & 10 (8\%) \\ 
 \bottomrule
\end{tabularx}
\newline
\label{table:pull_request_consequences}
\vspace{-6mm}
\end{table}

==> table/table-rq1-top-concerns.tex <==
\begin{table}[t]
\centering
\small
\caption{The identified security concerns in CWE-699 categories. The bold text indicates the top 10 concerns in each project. The ${\ddag}$ symbol indicates the concerns that were frequently raised in both OpenSSL and PHP.}
\begin{tabularx}{\linewidth}{
            >{\hsize=2.0\hsize}X
            >{\hsize=0.10\hsize}X
            >{\hsize=0.28\hsize}X |
            >{\hsize=0.10\hsize}X 
            >{\hsize=0.28\hsize}X
          }
\toprule
  \multirow{2}{*}{\textbf{Category (CWE-\#)}} & \multicolumn{2}{c|}{\textbf{OpenSSL}} & \multicolumn{2}{c}{\textbf{PHP}} \\
        & \# & \% & \# & \% \\
  \hline

    Authentication Errors (1211) \ddag&\textbf{21}&\textbf{11.17\%}&\textbf{9}&\textbf{7.32\%}\\
    API / Function Errors (1228) \ddag&\textbf{13}&\textbf{6.91\%}&\textbf{6}&\textbf{4.88\%}\\
    Random Number Issues (1213) \ddag&\textbf{13}&\textbf{6.91\%}&\textbf{5}&\textbf{4.07\%}\\
    Behavioral Problems (438 ) \ddag&\textbf{12}&\textbf{6.38\%}&\textbf{5}&\textbf{4.07\%}\\
    Resource Locking Problems (411)&\textbf{15}&\textbf{7.98\%}&3&2.44\%\\
    Cryptographic Issues (310) \ddag&\textbf{7}&\textbf{3.72\%}&\textbf{8}&\textbf{6.50\%}\\
    Audit / Logging Errors (1210)&5&2.66\%&\textbf{8}&\textbf{6.50\%}\\
    Initialization and Cleanup Errors (452)&\textbf{15}&\textbf{7.98\%}&1&0.81\%\\
    Concurrency Issues (557)&\textbf{9}&\textbf{4.79\%}&4&3.25\%\\
    Privilege Issues (265) \ddag&\textbf{7}&\textbf{3.72\%}&\textbf{5}&\textbf{4.07\%}\\
    Pointer Issues (465)&2&1.06\%&\textbf{8}&\textbf{6.50\%}\\
    Information Management Errors (199)&5&2.66\%&\textbf{6}&\textbf{4.88\%}\\
    Memory Buffer Errors (1218)&\textbf{7}&\textbf{3.72\%}&4&3.25\%\\
    Type Errors (136) &\multicolumn{2}{c|}{-}&\textbf{8}&\textbf{6.50\%}\\
    Resource Management Errors (399) &\multicolumn{2}{c|}{-}&\textbf{7}&\textbf{5.69\%}\\
    Business Logic Errors (840)&6&3.19\%&3&2.44\%\\
    Data Processing Errors (19)&6&3.19\%&2&1.63\%\\
    Communication Channel Errors (417) &\textbf{9}&\textbf{4.79\%}&\multicolumn{2}{c}{-}\\
    File Handling Issues (1219)&2&1.06\%&4&3.25\%\\
    Data Neutralization Issues (137) &\multicolumn{2}{c|}{-}&\textbf{5}&\textbf{4.07\%}\\
    Documentation Issues (1225) &\multicolumn{2}{c|}{-}&\textbf{5}&\textbf{4.07\%}\\
    String Errors (133)&1&0.53\%&4&3.25\%\\
    Handler Errors (429)&4&2.13\%&2&1.63\%\\
    Expression Issues (569) &\textbf{7}&\textbf{3.72\%}&\multicolumn{2}{c}{-}\\
    User Session Errors (1217)&2&1.06\%&3&2.44\%\\
    Data Integrity Issues (1214)&3&1.60\%&2&1.63\%\\
    Signal Errors (387)&2&1.06\%&2&1.63\%\\
    State Issues (371)&2&1.06\%&2&1.63\%\\
    Error Conditions, Return Values, ... (389) &4&2.13\%&\multicolumn{2}{c}{-}\\
    Permission Issues (275)&2&1.06\%&1&0.81\%\\
    Credentials Management Errors (255) &3&1.60\%&\multicolumn{2}{c}{-}\\
    Bad Coding Practices (1006) &2&1.06\%&\multicolumn{2}{c}{-}\\
    Data Validation Issues (1215)&\multicolumn{2}{c|}{-}&1&0.81\%\\
    Complexity Issues (1226) &1&0.53\%&\multicolumn{2}{c}{-}\\
    Key Management Errors (320) &1&0.53\%&\multicolumn{2}{c}{-}\\
    Authorization Errors (1212)&\multicolumn{2}{c|}{-}&\multicolumn{2}{c}{-}\\
    Encapsulation Issues (1227)&\multicolumn{2}{c|}{-}&\multicolumn{2}{c}{-}\\
    Lockout Mechanism Errors (1216)&\multicolumn{2}{c|}{-}&\multicolumn{2}{c}{-}\\
    Numeric Errors (189)&\multicolumn{2}{c|}{-}&\multicolumn{2}{c}{-}\\
    User Interface Security Issues (355)&\multicolumn{2}{c|}{-}&\multicolumn{2}{c}{-}\\
    
    
 \bottomrule
\end{tabularx}
\newline
\label{table:rq1_top_concerns}
\end{table}


==> table/table-test-models-recall.tex <==
\begin{table*}[ht!]
\centering
\caption{Recall scores at top K comments}
\begin{tabularx}{\linewidth}{
            >{\hsize=1.8\hsize}X
            >{\hsize=0.8\hsize}X
            >{\hsize=0.8\hsize}X
            >{\hsize=0.8\hsize}X
            >{\hsize=0.8\hsize}X
            >{\hsize=0.8\hsize}X
            >{\hsize=0.8\hsize}X
            >{\hsize=0.8\hsize}X
            >{\hsize=0.8\hsize}X
          }
\toprule
\multirow{2}{*}{Top K comments} &  \multicolumn{4}{c}{\textbf{OpenSSL}} & \multicolumn{4}{c}{\textbf{PHP}}\\
 \cline{2-9}
  & KW & NS & SC SO & SC Vul & KW & NS & SC SO & SC Vul\\
  \hline
 Recall at 20 &  \multirow{5}{*}{ 0.19048 } & 0.14286 & \textbf{0.20239} & 0.17857 & \multirow{5}{*}{ 0.19697 }  & 0.09091 & 0.19697 & \textbf{0.21212}\\
 Recall at 40 & & 0.25 & \textbf{0.30952} & 0.27381 & & 0.16667 & 0.27273 & \textbf{0.28787}\\
 Recall at 60 & & 0.36905 & \textbf{0.41667} & 0.36905 & & 0.22727 & 0.34848 & \textbf{0.40909} \\
 Recall at 80 & & 0.46428 & \textbf{0.5} & 0.45238 & & 0.33333 & 0.45454 & \textbf{0.53030} \\
 Recall at 100 & & 0.53571 & \textbf{0.59524} & 0.51190 & & 0.42424 & \textbf{0.60606} & 0.57576 \\
 \bottomrule
\end{tabularx}
\newline
\label{table:approach_selection}
\vspace{-6mm}
\end{table*}

==> table/table-tool-version.tex <==
\begin{table}[h]
\centering
\small
\caption{Versions of \SAT{s} used in this study}
\begin{tabularx}{\linewidth}{
            >{\hsize=1\hsize}X
            >{\hsize=1\hsize}X
          }
\toprule
\textbf{Tool Name} & \textbf{Version}\\
 \midrule
 \textbf{Cppcheck} & 2.10 \\ 
 \textbf{CodeChecker} & 6.22.2 \\ 
 \textbf{CodeQL} & 2.13.3 \\ 
 \textbf{Flawfinder} & 2.0.19 \\ 
 \textbf{Infer} & 1.1.0 \\
\bottomrule
\end{tabularx}
\newline
\label{table:tool-version}
\end{table}

==> table/table-warning-severity-mapping.tex <==
\begin{table}[h]
\centering
\small
\caption{\SATC{} warning severity}
\begin{tabularx}{\linewidth}{
            >{\hsize=1\hsize}X
            >{\hsize=1\hsize}X
            >{\hsize=1\hsize}X
          }
\toprule
\textbf{Tool} & \textbf{Original Severity} & \textbf{Mapped Severity }\\
 \hline 
 CodeChecker & Error & \multirow{5}*{High} \\
 CodeQL & Error &  \\
 CppCheck & High &  \\
 Infer & Error &  \\
 Flawfinder & Error &  \\
 \hline
 CodeChecker & Medium & \multirow{5}*{Medium} \\
 CodeQL & Warning &  \\
 CppCheck & Warning &  \\
 Infer & Warning, Advice &  \\
 Flawfinder & Warning &  \\
 \hline
 CodeChecker & Low & \multirow{5}*{Low} \\
 CodeQL & Note &  \\
 CppCheck & Information, Debug, Portability, Style, Performance, None &  \\
 Infer & Info, Like &  \\
 Flawfinder & Note &  \\
 
\end{tabularx}
\newline
\label{table:warning-severity-mapping}
\end{table}
